The Parallelism Motifs of Genomic Data Analysis

Genomic data sets are growing dramatically as the cost of sequencing continues to decline and small sequencing devices become available. Enormous community databases store and share this data with the research community, but some of these genomic data analysis problems require large scale computational platforms to meet both the memory and computational requirements. These applications differ from scientific simulations that dominate the workload on high end parallel systems today and place different requirements on programming support, software libraries, and parallel architectural design. For example, they involve irregular communication patterns such as asynchronous updates to shared data structures. We consider several problems in high performance genomics analysis, including alignment, profiling, clustering, and assembly for both single genomes and metagenomes. We identify some of the common computational patterns or motifs that help inform parallelization strategies and compare our motifs to some of the established lists, arguing that at least two key patterns, sorting and hashing, are missing.

==> tables/tab1.tex <==
\begin{table}[t]
	\centering
	\caption{\textbf{LOGAN} and \textbf{SeqAn} execution times in seconds for 100K alignments (POWER9 platform with 6 NVIDIA Tesla V100s).}
	\label{table:performance_comparison_1}
% 	\resizebox{\columnwidth}{!}{%
	\begin{tabular}{rrrr}
	\toprule
		\multirow{2}{*}{\textbf{$X$-Drop}} &\textbf{SeqAn}& \textbf{LOGAN} & \textbf{LOGAN} \\%& \textbf{Speed-Up}& \textbf{Speed-Up}\\
		 &\textbf{168 CPU Threads}& \textbf{1 GPU} & \textbf{6 GPU} \\%& \textbf{1 GPU} & \textbf{6 GPU} \\
	\midrule
	    10  & 5.1  &2.2 &1.9 \\%&2.3$\times$ & 2.7$\times$ \\ 
	\midrule
        20  & 12.7 &3.1 &2.1\\% &4.1$\times$ & 6.2$\times$ \\ 
    \midrule
        50 & 29.6  &5.0 &2.2 \\%\\%&6.0$\times$ & 13.2$\times$ \\ 
    \midrule
        100 & 45.7 &7.2 &2.7\\% &6.4$\times$ & 17.0$\times$ \\ 
    \midrule
        500& 102.6 &14.9&4.0\\% &6.9$\times$ & 25.9$\times$ \\  
    \midrule
        1000& 133.3 &20.2&4.9\\% &6.6$\times$ & 27.4$\times$ \\  
    \midrule
        2500& 168.0&25.3&5.6 \\%\\%&6.6$\times$ & 30.3$\times$ \\  
    \midrule
        5000 & 176.6 & 26.7 &5.8 \\%&6.6$\times$ & 30.7$\times$ \\ 		
	\bottomrule
	\end{tabular}%
% 	}
\end{table}

==> tables/tab2.tex <==
\begin{table}[t]

	\centering
	\caption{Execution times on ``POWER9'' platform with 6 NVIDIA Tesla V100s in seconds for 3.62M alignments ({\em A. baumannii}).\newline
	\textbf{BELLA} indicates the original software, while \textbf{LOGAN} indicates that BELLA uses LOGAN for alignment.}
	\label{table:performance_comparison_2}
	\resizebox{\columnwidth}{!}{%
\begin{tabular}{rrrrrr}
	\toprule
		\multirow{2}{*}{\textbf{$X$-Drop}} &\textbf{BELLA}& \textbf{LOGAN} & \textbf{LOGAN} & \textbf{Speed-Up}& \textbf{Speed-Up}\\
		 &\textbf{168 CPU Threads}& \textbf{1 GPU} & \textbf{6 GPU} & \textbf{1 GPU} & \textbf{6 GPU} \\
	\midrule
	    5 &  52.20 & 123.12 & 109.81 & 0.4$\times$ & 0.5$\times$ \\ 
	\midrule
        10 & 106.55 & 129.07 & 111.01 & 0.8$\times$ & 1.0$\times$ \\ 
    \midrule
        15 & 170.43 & 135.48 & 113.18 & 1.3$\times$ & 1.5$\times$ \\ 
    \midrule
        20 & 222.34 & 142.39 & 114.90 & 1.6$\times$ & 1.9$\times$ \\ 
    \midrule
        25 & 270.02 & 149.87 & 116.92 & 1.8$\times$ & 2.3$\times$ \\  
    \midrule
        30 & 309.54 & 157.93 & 117.27 & 2.0$\times$ & 2.6$\times$ \\  
    \midrule
        35 & 346.35 & 166.65 & 119.51 & 2.1$\times$ & 2.9$\times$ \\  
    \midrule
        40 & 379.67 & 176.06 & 121.38 & 2.2$\times$ & 3.1$\times$ \\ 
    \midrule
        50 & 440.45 & 186.23 & 122.25 & 2.4$\times$ & 3.6$\times$ \\ 
    \midrule
        80 & 584.32 & 197.20 & 124.79 & 3.0$\times$ & 4.7$\times$ \\
    \midrule
        100 & 666.11 & 219.75 & 126.74 & 3.0$\times$ & 5.3$\times$ \\
	\bottomrule
	\end{tabular}%
	}
\end{table}

==> tables/tab3.tex <==
\begin{table}[t]
	\centering
	\caption{Execution times on POWER9 platform with 6 NVIDIA Tesla V100s in seconds for 1.82M alignments ({\em E. coli}).}
	%\newline
	%\textbf{BELLA} indicates the original software, while \textbf{LOGAN} indicates that BELLA uses LOGAN for alignment.}
	\label{table:performance_comparison_3}
% 	\resizebox{\columnwidth}{!}{%
	\begin{tabular}{rrrr}
	\toprule
		\multirow{2}{*}{\textbf{$X$-Drop}} &\textbf{BELLA}& \textbf{LOGAN} & \textbf{LOGAN}\\ % & \textbf{Speed-Up}& \textbf{Speed-Up}\\
		 &\textbf{168 CPU Threads}& \textbf{1 GPU} & \textbf{6 GPU} \\% & \textbf{1 GPU} & \textbf{6 GPU} \\
	\midrule
	    5 &  53.2 & 110.4 & 114.3 \\ %& 0.48$\times$ & 0.47$\times$\\ 
	\midrule
        10 &108.6 & 146.4 & 115.3 \\ %& 0.74$\times$ & 0.94$\times$\\ 
    \midrule
        15 &139.0 & 152.9 & 114.8 \\ %& 0.91$\times$ & 1.21$\times$\\ 
    \midrule
        20 &226.7 & 162.7 & 118.4 \\ % & 1.39$\times$ & 1.91$\times$\\ 
    \midrule
        25 &275.3 & 173.5 & 125.3 \\ %& 1.59$\times$ & 2.20$\times$\\  
    \midrule
        30 &558.0 & 185.3 & 130.6 \\%& 3.01$\times$ & 4.27$\times$\\  
    \midrule
        35 &654.1 & 198.4 & 136.8 \\ %& 3.30$\times$ & 4.78$\times$\\  
    \midrule
        40 &750.1 & 212.7 & 138.4 \\ %& 3.53$\times$ & 5.42$\times$\\ 
    \midrule
        50 &913.1 & 248.5 & 141.4 \\%& 3.67$\times$ & 6.41$\times$\\ 
    \midrule
        80 &1303.7 & 295.8 & 142.4 \\%& 4.41$\times$  & 9.03$\times$ \\
    \midrule
        100 & 1507.1 & 336.3 & 144.5 \\%& 4.48$\times$  & 10.66$\times$ \\
	\bottomrule
	\end{tabular}%
% 	}
\end{table}

==> tables/tab4.tex <==
\begin{table}[t]
	\centering
	\caption{\textbf{LOGAN} and \textbf{ksw2} execution times in seconds for 100K alignments (``Skylake'' platform with 8 NVIDIA Tesla V100s).}
	\label{table:performance_comparison_4}
% 	\resizebox{\columnwidth}{!}{%
	\begin{tabular}{rrrr}
	\toprule
		\multirow{2}{*}{\textbf{$X$-Drop}} &\textbf{ksw2}& \textbf{LOGAN} & \textbf{LOGAN} \\%& \textbf{Speed-Up}& \textbf{Speed-Up}\\
		 &\textbf{80 CPU Threads}& \textbf{1 GPU} & \textbf{8 GPU }\\%\\% & \textbf{1 GPU} & \textbf{8 GPU} \\
	\midrule
	    10  & 6.9 & 2.5 & 1.7 \\%& 2.8$\times$ & 4.1$\times$ \\ 
	\midrule
        20  & 7.0 & 3.8 & 1.8 \\%\\%\\%\\%\\%\\%\\%& 1.8$\times$ & 3.9$\times$ \\ 
    \midrule
        50 & 7.7 & 5.8 & 2.1 \\%\\%\\%\\%\\%\\%& 1.3$\times$ & 3.6$\times$ \\ 
    \midrule
        100 & 10.4 & 7.3 & 2.4 \\%\\%\\%\\%\\%& 1.4$\times$ & 4.3$\times$ \\ 
    \midrule
        500 & 113.0 & 15.2 & 3.4 \\%\\%\\%\\%& 7.4$\times$ & 33.1$\times$ \\  
    \midrule
        1,000& 209.5 & 20.4 & 4.3 \\%\\%\\%& 10.3$\times$ & 48.3$\times$ \\  
    \midrule
        2,500& 1235.8 & 25.9 & 5.2 \\%\\%& 47.8$\times$ & 238.6$\times$ \\  
    \midrule
        5,000& 3213.1 & 27.2 & 5.2 \\%& 118.1$\times$ & 614.4$\times$ \\ 		
	\bottomrule
	\end{tabular}%
% 	}
\end{table}

==> tables/tab5.tex <==
\begin{table}[t]
    \centering
    \caption{$X$-drop execution times on GPU using $X=100$ and exploiting different levels of parallelism.}
    \label{table:parallel}
    \resizebox{\columnwidth}{!}{%
	\begin{tabular}{lrrrrrr}
	\toprule
	 \multicolumn{1}{c}{\textbf{Parallelism}} &
    \multicolumn{1}{c}{\textbf{Pairs}}  & \multicolumn{1}{c}{\textbf{Threads}} & \multicolumn{1}{c}{\textbf{Blocks}}  & \multicolumn{1}{c}{\textbf{Time}} &
    \multicolumn{1}{c}{\textbf{Speed-Up}}\\
    \midrule
    None & 1 & 1 & 1 & 1.50s & - \\
    \midrule
    Intra-sequence & 1 & 128 & 1 & 0.16s & 9.3$\times$ \\
    \toprule
    Intra-sequence & 100K & 128 & 1 & 45h & - \\
    \midrule
    Intra- and inter-sequence & 100K & 128 & 100K & 7.35s & 22000.0$\times$ \\
    \bottomrule
    \end{tabular}%
    }
\end{table}

==> tables/tab6.tex <==
\begin{table}[t]
	\centering
	\caption{Execution times on POWER9 platform with 6 NVIDIA Tesla V100s in seconds for 235M alignments ({\em C. elegans}).}%\newline
% 	\textbf{BELLA} indicates the original software, while \textbf{LOGAN} indicates that BELLA uses LOGAN for alignment.}
	\label{table:performance_comparison_2}
% 	\resizebox{\columnwidth}{!}{%
	\begin{tabular}{rrrr}
	\toprule
		\multirow{2}{*}{\textbf{$X$-Drop}} &\textbf{BELLA}& \textbf{LOGAN} & \textbf{LOGAN}\\ % & \textbf{Speed-Up}& \textbf{Speed-Up}\\
		 &\textbf{168 CPU Threads}& \textbf{1 GPU} & \textbf{6 GPU} \\% & \textbf{1 GPU} & \textbf{6 GPU} \\
	\midrule
	    5 & 131.7 & 577.1 & 213.1 \\ %& 0.48$\times$ & 0.47$\times$\\ 
	\midrule
        10 & 723.3 & 750.2 & 579.7 \\ %& 0.74$\times$ & 0.94$\times$\\ 
    \midrule
        15 & 1467.7 & 865.6 & 749.8 \\ %& 0.91$\times$ & 1.21$\times$\\ 
    \midrule
        20 & 1954.8 & 908.9 & 777.0 \\ % & 1.39$\times$ & 1.91$\times$\\ 
    \midrule
        25 & 2518.8 & 1015.5 & 838.9 \\ %& 1.59$\times$ & 2.20$\times$\\  
    \midrule
        30 & 3047.1 & 1125.0 & 888.0 \\%& 3.01$\times$ & 4.27$\times$\\  
    \midrule
        35 & 3492.5 & 1226.5 & 927.0 \\ %& 3.30$\times$ & 4.78$\times$\\  
    \midrule
        40 & 3887.0 & 1329.0 & 955.9 \\ %& 3.53$\times$ & 5.42$\times$\\ 
    \midrule
        50 & 4607.7 & 1449.0 & 983.7 \\%& 3.67$\times$ & 6.41$\times$\\ 
    \midrule
        80 & 6367.7 & 1593.9 & 1046.1 \\%& 4.41$\times$  & 9.03$\times$ \\
    \midrule
        100 & 7385.3 & 1753.3 & 1080.9 \\%& 4.48$\times$  & 10.66$\times$ \\
	\bottomrule
	\end{tabular}%
% 	}
\end{table}

%GIULIA: leave .9 to have values alignment in the table
